Harpocrates: Anonymous Data Publication in Named Data Networking

Named-Data Networking (NDN), a prominent realization of the Information-Centric Networking (ICN) vision, offers a request-response communication model where data is identified based on application-defined names at the network layer. This amplifies the ability of censoring authorities to restrict user access to certain data/websites/applications and monitor user requests. The majority of existing NDN-based frameworks have focused on enabling users in a censoring network to access data available outside of this network, without considering how data producers in a censoring network can make their data available to users outside of this network. This problem becomes especially challenging, since the NDN communication paths are symmetric, while producers are mandated to sign the data they generate and identify their certificates. In this paper, we propose Harpocrates, an NDN-based framework for anonymous data publication under censorship conditions. Harpocrates enables producers in censoring networks to produce and make their data available to users outside of these networks while remaining anonymous to censoring authorities. Our evaluation demonstrates that Harpocrates achieves anonymous data publication under different settings, being able to identify and adapt to censoring actions.

==> Sections/motivation.tex <==
\section {Motivation and Challenges}
\label{sec:motivation}

Let us consider authorities such as governments, ISPs, and organizations that actively monitor, intercept, and inspect the communications and the network traffic of their citizens/users. In addition, such authorities may restrict their citizens/users from accessing websites and data (content) that they do not consider favorable as well as identify and hold accountable citizens/residents that upload non-favorable data on the Internet. For example, during protests in a certain country, protesters may take pictures or videos that show law enforcement personnel attempting to violently suppress these protests. The government may restrict the protesters from uploading this data to popular hosting websites (\eg YouTube and Vimeo), news websites (\eg CNN and BBC), and social media platforms (\eg Facebook and Instagram). Such a measure aims to prevent the data from being accessible by users on the public Internet, since this would essentially reveal the reality about the protests and their suppression to the rest of the world. However, in cases that users find ways to evade censorship and upload their data on the public Internet (\eg by uploading the data on websites not blocked by the country's government), the government in cooperation with local ISPs may be able to identify the citizen(s) that uploaded the data and imprison them. Subsequently, hosting, news, and social media websites have vested interest in verifying the authenticity of the uploaded data before making it available to their users without compromising the producer anonymity.

This scenario showcases the main motivation behind the design of \sol, which aims to tackle the following questions: 
%
%\begin{itemize}[leftmargin=*]
{\it (i) How can citizens/users that produce data within oppressive countries and organizations (censoring networks) publish this data on the public Internet (non-censoring networks)?
and (ii) How can the produced data be published and authenticated on the public Internet while its producers remain anonymous to the oppressive countries and organizations, which could threaten the producers' safety and well-being?}
%\end{itemize}
%
Note that \sol focuses on anonymous publication of data produced within censoring networks, which involves data production, uploading, and sharing with users outside of these networks, rather than simply evading censorship to access (download) data from websites blocked within censoring networks. 

{\spyros Today, public key certificates are used to prove that a user is the owner of a specific pair of public-private keys. Such certificates are used to authenticate users and, as a consequence, the data they produce. However, a certificate may include and reveal information about the identity of its owner (at the very least, the owner's email address). In NDN, producers sign each packet of generated data, which carries the resulting signature at the network layer. This signature is used by requesters to authenticate the received packets. However, each packet of data contains signature related information that identify the producer's certificate~\cite{ndn2015ndn}, which may reveal information about the producer linking the data back to the producer. %NDN/ICN may not contain source and destination addresses in their packets. 
Furthermore, the following NDN architectural features can facilitate the ability of censoring authorities to impose communication restrictions:}

%, being able to provide only up to a certain level of anonymity depending on how sensitive the included identity information is.

%{\abde I think it is very verbose for a challenge that we don't address ``complete'' in this paper. I suggest that at least we remove the NDN part since this challenge is also an IP challenge.} {\reza I didn't get the third sentence starting with ``However, certificates ... ''}

\begin{enumerate}[leftmargin=*]

\item The use of application-defined (and semantically meaningful in particular in the case of NDN) naming for communication purposes at the network layer directly reveals the requested data to censoring authorities. As a result, requests for non-favorable data can be easily blocked by censoring authorities.

\item The NDN/ICN communication model itself is requester-initiated and symmetric. In other words, the requested data will follow the same network path back to the requester as its corresponding request. In such cases, even if a request is not blocked by censoring authorities based on the name of the requested data, the request can be analyzed and the corresponding response can be blocked on its way back to the requester.

%\item Each producer is mandated to sign each packet of generated data, which carries the resulting signature at the network layer. Each packet of data also contains signature related information that reveals the producer's certificate or public key~\cite{ndn2015ndn}, so that requesters can authenticate the received packets. %{\spyros However, it also creates strong linkability between the producer's identity (a public-key certificate) and its data~\cite{ellison2000ten, garfinkel2003email}}. %{\abde This bullet maybe removed entirely. Or simply change it to say: While NDN hides the source of the data (no IP addresses used), it mandates signing all data packets compared to IP architecture (\eg signature used on TLS initialization).} {\reza I would suggest removing the blue part and simply saying it reveals producer's certificate. Also, the part Abde mentioned makes sense.}

\item As a by-product of (1) and (2), producers in censoring networks: (i) cannot advertise the data they produce, since this would enable censoring authorities to directly link the generated data to them; and (ii) cannot be reachable from outside of censoring networks, since censoring authorities can easily drop incoming requests with non-favorable or unknown data names.

\end{enumerate}

For all these reasons, anonymously publishing data produced within censoring networks is particularly challenging in NDN/ICN and cannot be supported by the native features of such a data-centric architecture. To tackle these challenges, we propose \sol, a framework that extends the NDN architecture for the anonymous publication of data produced within censoring networks. To the best of our knowledge, \sol is the first of its kind in NDN/ICN research. As we further discuss in Section~\ref{subsec:related-work}, several prior works in NDN/ICN have considered evading censorship to retrieve data available in non-censoring networks from within censoring networks~\cite{DibGasTsu11, ChuKimJan14, TouMisKli15, LesYaqKha19}. However, none of these works has considered cases of anonymously making data produced within censoring networks available outside of these networks, a scenario that occurs when data produced within oppressive countries or organizations needs to be made available on the public Internet.
